Probing the Unknown: Exploring Student Interactions with Probeable Problems at Scale in Introductory Programming

Introductory programming courses often rely on small code-writing exercises that have clearly specified problem statements. This limits opportunities for students to practice how to clarify ambiguous requirements -- a critical skill in real-world programming. In addition, the emerging capabilities of large language models (LLMs) to produce code from well-defined specifications may harm student engagement with traditional programming exercises. This study explores the use of ``Probeable Problems'', automatically gradable tasks that have deliberately vague or incomplete specifications. Such problems require students to submit test inputs, or `probes', to clarify requirements before implementation. Through analysis of over 40,000 probes in an introductory course, we identify patterns linking probing behaviors to task success. Systematic strategies, such as thoroughly exploring expected behavior before coding, resulted in fewer incorrect code submissions and correlated with course success. Feedback from nearly 1,000 participants highlighted the challenges and real-world relevance of these tasks, as well as benefits to critical thinking and metacognitive skills. Probeable Problems are easy to set up and deploy at scale, and help students recognize and resolve uncertainties in programming problems.

==> qualitative-analysis/version2.tex <==
We conducted a reflexive thematic analysis~\cite{clarke2017thematic} to understand students' perceptions of this type of task.  Students were asked to respond to the following question: \emph{``Please comment on your experience solving this type of `Ask the client' task (where you must create input tests to clarify the behavior of a vague problem statement before you can write code) compared to a more traditional programming task where a complete and detailed specification is provided to you.''}

Our thematic analysis revealed four key themes: aversion toward ambiguity, real-world relevance, learning benefits and enjoyment, and strategy and problem-solving. Each theme reflects different aspects of how students experienced these tasks.

\subsubsection{Difficulty and Frustration}

The most frequently cited theme (436 responses) was the difficulty and frustration that students experienced when completing the tasks. Many students found the vague problem descriptions and hidden requirements to be challenging. They often felt overwhelmed by the need to identify edge cases and account for unanticipated scenarios. One student noted, \textit{``I find these tasks often quite difficult because of how vague the question is. This means that I have to think ahead of time to determine different variables and how each of the sections of code will be laid out.''} Another remarked, \textit{``I struggled a lot when trying to find what the client is asking for. Once I found out what was being asked, I solved it, but there were things I forgot to check such as what if there is no evens.''}  

% A value related to wasting time. 

\subsubsection{Real-World Relevance}

A significant portion of students (348 responses) appreciated the alignment of these tasks with real-world programming scenarios. Many recognized that working with vague specifications and clarifying requirements mirrors the challenges faced by developers interacting with clients in professional contexts. One student commented, ``I enjoyed it; I thought it was more accurate to real-life examples where the client is not a coder and cannot describe the code that well but can give examples of exactly what they like.'' Another wrote, ``This type of exercise mimics a situation where a client asks the programmer to create a program in a vague manner. It makes me think consciously through every possible scenario and what the output of the program should be.''

%\begin{quote}
%    \textit{``It is hard to code not knowing exactly what the client wants, I can only imagine how hard it must be going back and forth with an actual client to make something for them.'' (P991)}
%\end{quote}

\subsubsection{Learning Benefits}

Responses (242) emphasized the learning opportunities provided by these tasks. Students highlighted that the process of probing for requirements and addressing edge cases deepened their understanding of programming concepts and problem-solving strategies. For example, a student shared, ``These tasks helped me think more deeply about the problem and discover aspects of the specification instead of just having it provided to me.'' Another remarked, ``It was frustrating at times, but it helped me improve my problem-solving skills and learn how to communicate better in code.'' 

%\subsection{Preference for Traditional Tasks}
\subsubsection{Aversion to Task Ambiguity}

Many students (312 responses) expressed a preference for traditional programming tasks with detailed specifications. They found these tasks more straightforward and less time-consuming, especially when they were struggling with the ambiguity of the `Ask the Client' format. One student stated, \textit{``I much prefer traditional programming tasks where it is less guessing what is wanted. With the 'Ask the Client' tasks, it is very easy to forget certain edge cases, which can be frustrating.''} Another commented, \textit{``I prefer a more detailed task because it’s easier to know exactly what is required of me.''} Students also frequently talked about the `time wasted' by requirement elicitation: 

\begin{quote}
\textit{``It can be a bit of a pain due to the lack of information provided from the client...The different interpretations can lead to going down many rabbit holes and causing time to be wasted.'' }    
\end{quote}

This was further reflected by other students as well who tended to blame the client and had the expectation that requirement elicitation was not a skill they needed to develop. For example, one participant stated,  

\begin{quote}
\textit{``The `ask the client' really shows WHAT NOT TO DO as a client or stakeholder. In reality, the client should provide a full list of requirements of what to achieve, or they should provide more details on a specific component''}
\end{quote}

This sentiment was succintly summarized by other participant saying simply, \textit{``I hate clients that aren't clear about what they want!''}. 

% \subsection{Enjoyment or Engagement}

% Despite the challenges, 247 responses indicated that students enjoyed or felt engaged by the tasks. They appreciated the novelty and problem-solving aspects, with some finding the process of uncovering requirements and handling edge cases intellectually stimulating. One student noted, ``I enjoyed these tasks; they are a good way to remember to make sure I am testing for edge cases and fully understand what the code is supposed to do.'' Another said, ``I really like these questions! They challenge me to think critically and improve my ability to look for edge cases.''

\subsection{Strategies and Problem-Solving}

Finally, 198 responses highlighted the strategies students developed to tackle the `Ask the Client' tasks. Many shared their approaches for identifying edge cases, systematically testing inputs, and iterating on their solutions. One student explained, ``I found it quite important to begin by trying all the potential input cases to see what the expected output should be so I got an idea of how to handle boundary cases and typical inputs.'' Another reflected, ``I learned to be more critical in finding possible edge cases to test. In future tasks, I will brainstorm edge cases before starting to code.''

% Overall, the thematic analysis revealed a spectrum of responses, ranging from frustration and difficulty to appreciation of real-world relevance and intellectual engagement. While many students found the tasks challenging, they also recognized the value of developing skills that are essential in professional programming contexts.

